Algorithms for Detecting Shape Defects in Concentrated Solar Power Plant Components

Concentrated solar power (CSP) technology offers a dispatchable renewable energy solution, capable of bridging the gap between intermittent generation and grid demand through high-capacity thermal energy storage. However, the overall thermodynamic efficiency and cost-effectiveness of CSP plants depend crucially on the optical quality and precise geometric alignment of thousands of reflective surfaces spread across vast solar fields. Shape defect detection algorithms have become essential tools for automating mirror profilometry, tracking the flow spot and diagnosing alignment issues. This paper presents a novel framework for geometric shape detection techniques tailored to CSP applications. It introduces the notion of \emph{parabolicity}, which motivates a class of optimisation problems in this setting and suggests a possible direction for further work in computational geometry. Both exact and approximate algorithms are proposed, together with an experimental study on synthetic datasets generated via simulation.

==> binning.tex <==
\begin{tikzpicture}


% Axes
\draw[->] (-2,0) -- (5,0) node[right] {$x$};
%\draw[->] (0,-0.5) -- (0,4) node[above] {$y$};
\fill[gray!50] (-1.5,0.7521798082800956) circle (2pt);
\fill (-1.25,0.85487737496677072) circle (2pt);
\fill[gray!50] (-1,0.521121668944425488) circle (2pt);
\fill[gray!50] (-0.75,0.2772977190515488) circle (2pt);
\draw[-,dashed,gray] (-0.625,0) to (-0.625,5);
\fill[gray!50] (-0.5,0.188314526079406976) circle (2pt);
\fill (-0.25,0.78124670434347856) circle (2pt);
\fill[gray!50] (0,0.026704143208924424) circle (2pt);
\fill[gray!50] (0.25,0.5186781749952676) circle (2pt);
\draw[-,dashed,gray] (0.375,0) to (0.375,5);
\fill[gray!50] (0.5,0.230885621241179976) circle (2pt);
\fill (0.75,0.53692959513043336) circle (2pt);
\fill[gray!50] (1,0.432468385723237248) circle (2pt);
\fill[gray!50] (1.25,0.249779440403177408) circle (2pt);
\draw[-,dashed,gray] (1.375,0) to (1.375,5);
\fill[gray!50] (1.5,0.72911398670466656) circle (2pt);
\fill[gray!50] (1.75,0.4217519973775552) circle (2pt);
\fill[gray!50] (2,0.89253101697838576) circle (2pt);
\fill (2.25,1.04794707641108936) circle (2pt);
\draw[-,dashed,gray] (2.375,0) to (2.375,5);
\fill (2.5,1.54595108711178896) circle (2pt);
\fill[gray!50] (2.75,1.3759216259430404) circle (2pt);
\fill[gray!50] (3,1.164281345741049288) circle (2pt);
\fill[gray!50] (3.25,1.53572032848500256) circle (2pt);
\draw[-,dashed,gray] (3.375,0) to (3.375,5);
\fill[gray!50] (3.5,1.666638667454948576) circle (2pt);
\fill[gray!50] (3.75,2.36170216712769192) circle (2pt);
\fill (4,2.62022367438137152) circle (2pt);
\draw[-,dashed,gray] (4.375,0) to (4.375,5);

\coordinate (punto) at (1.875,0);
\node [below] at (punto) {$I_j$};


\coordinate (puntob) at (0.875,0);
\node [below] at (puntob) {$I_{j-1}$};

\coordinate (puntobb) at (-0.275,0);
\node [xshift= 5, yshift= -10pt] at (puntobb) {$\dots$};


\coordinate (puntoa) at (2.875,0);
\node [below] at (puntoa) {$I_{j+1}$};

\coordinate (puntoaa) at (3.875,0);
\node [yshift = -10pt] at (puntoaa) {$\dots$};
\end{tikzpicture}


==> discarded.tex <==
\subsection{Defining the parabolicity}

In cases where the orientation is unknown, the complexity of this problem becomes significantly higher. The generic definition of this parabola in a plane is as follows:
\begin{equation} \label{conic}
    Ax^2 + Bxy + Cy^2 +Dx+Ey +F=0 
\end{equation}
With $B^2=4AC$.

If we wish to solve the same problem as expressed above, then the corridor is given by constants $F_1$, $F_2$ such that:
\begin{equation}
    F_2 \leq Ax_k^2+Bx_ky_k+Cy^2_k+Dx_k+Ey_k \leq F_1 \quad \text{for all } (x_k,y_k) \in \mathbb{R}^2
\end{equation}
Again, under the condition that $B^2=4AC$. With proper scaling, this can be simplified to a problem with six unknown values, $2n$ linear constraints, and a non-linear constraint. It becomes necessary, then, to add approximations to reduce the complexity of this problem.

Consider the family of conics (\ref{conic}), that satisfy $B^2-4AC=0$, normalized under the following condition:

\begin{equation}
    A^2 + B^2 + C^2 + D^2 + E^2 = 1
\end{equation}

Let us define then:
\begin{equation}
Q_\theta(x,y) = Ax^2 + Bxy + Cy^2 + Dx + Ey,
\quad \theta = (A,B,C,D,E)
\end{equation}

And for each point $(x_k,y_k)$, define the function $g_i(\theta)$: 
\begin{equation}
    g_k(\theta) = -Q_\theta(x_k,y_k)
\end{equation}

\begin{definition}[Parabolicity for non-oriented frameworks]
    Let $\mathcal{P} = \{(x_k,y_k)\}_{k=1}^n \subset \mathbb{R}^3$ be a finite set of points.
    Given $\theta$, our minimal-width parabolic corridor can be defined by the following identity:
\begin{equation}\label{deltaProof}
    \rho(\theta) = \max_{1 \le k \le n} g_k(\theta) - \min_{1 \le k \le n} g_k(\theta)
\end{equation}

From this, we can formulate the following optimization problem:
\begin{equation}\label{parabolicty:formulation}
\rho^*=\min_{\theta \in P} \rho(\theta),
\quad \text{where }
\Omega = \{\theta : B^2 - 4AC = 0,\; A^2 + B^2 + C^2 + D^2 + E^2 = 1\}
\end{equation}
We will say $\rho^*$ is the \textbf{parabolicity} of the point set $\mathcal{P}$.
\end{definition}

We can warrant the general existence of said minimal-width corridor, by using the following argument. 

\begin{lemma}[Existence of the parabolicity]
    The problem in (\ref{parabolicty:formulation}) has a global solution.
\end{lemma}

\begin{proof}First, we define the space where we search for our minimizing $\theta$. On one hand, the set of normalized $\theta$ can also be expressed as follows:
\begin{equation}
    S = \{(A,B,C,D,E) \in \mathbb{R}^5 : A^2 + B^2 + C^2 + D^2 + E^2 = 1\}
\end{equation}
This is, in fact, a compact set in $\mathbb{R}^5$ as it corresponds to the unit sphere of the Euclidean norm. On the other hand, $\mathcal{B} = \{\theta \in \mathbb{R}^5: B^2-4AC=0\}$ is closed in $\mathbb{R}^5$. Therefore, $\Omega = S \cap \mathcal{B}$ and $\Omega$ is compact.
Now, we use the fact that $g_k(\theta):\theta \longmapsto -Q_\theta(x_k,y_k)$ is continuous over $\theta$ given $k$. If we define the functions:
\begin{equation}
    \theta \mapsto \max_k g_k(\theta), \quad \theta \mapsto \min_k g_k(\theta)
\end{equation}
These will also be continuous, as we are working with a finite set of points $\{ (x_y,y_k) \}_k$, and $\delta(\theta)$ as defined in (\ref{deltaProof}) is continuous on $P$.

Since $\rho(\theta)$ is continuous and $P$ is compact, Weierstrass' theorem ensures that there exists a $\theta^*$ such that:
\begin{equation} \label{eq:parabolicityGeneral}
    \rho(\theta^*) = \min_{\theta \in \Omega} \rho(\theta)
\end{equation}
Which corresponds to the minimum width corridor defined between two parabolas displaced along their axis of symmetry, or as we defined earlier, the parabolicity of the finite point set $\{(x_k,y_k)\}_k$.
\end{proof}


As defined in (\ref{eq:parabolicityGeneral}), this problem is non-convex and not easily solved without approximations. It is reminiscent of the problem of cylindricity, yet with the added complexity of the condition $B^2-4AC=0$, which cannot be easily approximated without changing the geometry of the problem we are solving.

\begin{lemma}[Monotonicity with respect to the observations] \label{monotonicity}
Let $\mathcal{P}_1$ and $\mathcal{P}_2$ be two sets of points such that $\mathcal{P}_1 \subseteq \mathcal{P}_2$, and let $\theta \subseteq S$ a closed set denote the same admissible parameter set for both problems:
\begin{equation*}
\rho^*(\mathcal{P},\Theta)
=
\min_{\theta\in\Theta}
\left\{
\max_{k\in \mathcal{P}} g_k(\theta)
-
\min_{k\in \mathcal{P}} g_k(\theta)
\right\}
\end{equation*}
Then
\begin{equation*}
\rho^*(\mathcal{P}_1,\Theta)\leq \rho^*(\mathcal{P}_2,\Theta)
\end{equation*}

\end{lemma}

\begin{proof}
For every fixed $\theta\in\Theta$, since $\mathcal{P}_1 \subseteq \mathcal{P}_2$,
\begin{equation*}
\max_{k\in \mathcal{P}_1} g_k(\theta)
\leq
\max_{k\in \mathcal{P}_2} g_k(\theta),
\end{equation*}
while
\begin{equation*}
\min_{k\in \mathcal{P}_1} g_k(\theta) \geq
\min_{k\in \mathcal{P}_2} g_k(\theta)
\end{equation*}
Therefore,
\begin{equation*}
\max_{k\in \mathcal{P}_1} g_k(\theta)
-
\min_{k\in \mathcal{P}_1} g_k(\theta)
\leq
\max_{k\in \mathcal{P}_2} g_k(\theta)
-
\min_{k\in \mathcal{P}_2} g_k(\theta)
\end{equation*}
for every $\theta\in\Theta$. Taking the minimum over the same set $\Theta$ on both sides yields:
\begin{equation*}
\rho^*(\mathcal{P}_1,\Theta)\leq \rho^*(\mathcal{P}_2,\Theta).
\end{equation*}
\end{proof}

\begin{lemma}[Two boundaries on parabolicity] \label{boundaries_parabolicity}
Let $\mathcal{P}$ be a finite point set, let $\Theta$ be an admissible parameter set, and write $\rho^*=\rho^*(\mathcal{P},\Theta)$:
\begin{enumerate}
    \item For every subset $\mathcal{S} \subset \mathcal{P}$,
    \begin{equation*}
        \rho_{lower} := \rho^*(\mathcal{S},\Theta) \leq \rho^*
    \end{equation*}
    \item For every admissible $\theta \in \Theta$,
    \begin{equation*}
        \rho_{upper} :=  \max_{k\in\mathcal{P}}{g_k(\theta)} - \min_{k\in\mathcal{P}}{g_k(\theta)} \geq \rho^*
    \end{equation*}
\end{enumerate}
In particular, $\rho_{lower} \leq \rho  \leq \rho_{upper} $, and when $\theta$ is chosen to be the optimal argument of the problem on $\mathcal{S}$, then both boundaries are obtained from a single solve on $\mathcal{S}$, followed by a computation of $g_k$ over the points of $\mathcal{P}$.
\end{lemma}

\begin{proof}
The first part is given by applying Lemma \ref{monotonicity} to the sets $\mathcal{S}\subset\mathcal{P}$. The second assumption is given by the fact that $\theta$ is feasible for the problem that defines $\rho^*$, so by definition, the value of the objective function on $\theta$ will always be bounded below by the minimum. 
\end{proof}

There is a certain usefulness to this result, since it can be used to define a tolerance of the values we use in case points are discarded. That is, if for a given point cloud $\mathcal{P}$ we select a subset of these points, for whichever reason, we can solve the linear problem of parabolicity as stated in (\ref{eq:lp1}) and obtain the tolerance $\rho_{upper} -\rho_{lower}$ to determine how good of an approximation it is, without knowing the real parabolicity $\rho^*$.


It is also worth mentioning that, under experimental conditions, the angle $\theta$ can be refined to an interval $\theta \in [-\varphi,\varphi]$, as we will see in later sections.

We can, in fact, prove that the algorithm we just presented constitutes a $(1+\varepsilon)$-approximation.

\begin{theorem}[The rotation search is a $(1+\varepsilon)$-approximation]
    Let $\mathcal{P}$ be a finite point set of radius $R=max_k\|p_k\|$ about the pivot of rotations; let $I$ be a closed interval of axis directions that satisfy the hypothesis of Lemma \ref{rotformulation}, and 
    \begin{equation*}
        \rho^*_I = \min_{\varphi \in I}{w(\varphi)}
    \end{equation*}
    Suppose the optimal coefficients satisfy that $|a|, |b| \leq \kappa$ $\forall \varphi \in I$, and define:
    \begin{equation*}
        L = 2(R+\kappa R+2\kappa R^2)
    \end{equation*}
    Let $\varphi_1 <\dots <\varphi_m$ be a finite subset of $I$ of spacing at most $h$, and let $\tilde{\rho} = \min_{1\leq j \leq m} {w(\varphi_j)}$ be the parabolicity obtained by the rotational search. Then:
  \begin{equation}
      \rho^*_I \leq \rho \leq \rho^*_I + \frac{1}{2}Lh
  \end{equation}  
  Which, for a small enough $h$, becomes:
    \begin{equation} \label{approx:eq}
      \rho^*_I \leq \rho \leq (1+\varepsilon) \rho^*_I 
  \end{equation}  
\end{theorem}

\begin{proof}
    The left-hand side of the (\ref{approx:eq}) is given using Lemma \ref{boundaries_parabolicity}, since the rotational parabolicity is evaluated over a subset of parameters (angles) of $I$. 
    For the other inequality, we prove that $w$ is L-Lipchitz continuous.

    Given $\varphi, \psi \in I$ so that $\psi$ is the optimal in the interval $(a,b)$, that is, $w(\psi)=\text{rg}(r(\psi;a,b))$, while $w(\varphi) \leq \text{rg}(r(\varphi;a,b))$. Now, we work with the components of each point vector $p_k(\cdot)=(x_k(\cdot),y_k(\cdot))$. Since $p_k$ experiences a rotation, by definition we know all components $x_k(\varphi), y_k(\varphi), \partial_\varphi x_k(\varphi)$ and $\partial_\varphi y_k(\varphi)$ are bounded by $R$ and since:
    \begin{equation*}
        \frac{\partial r_k}{\partial \varphi}(\varphi) = \partial_\varphi y_k (\varphi) - 2a x_k(\varphi) \partial_\varphi x_k (\varphi) - b \partial_\varphi x_k(\varphi)   \end{equation*}
    Then we it follows that:
    \begin{equation*}
        \left| \frac{\partial r_k}{\partial \varphi} \right| \leq R + 2 |a|R^2 + |b| \leq R + 2\kappa R^2 + \kappa R = \frac{L}{2}
    \end{equation*}
    Uniformly in $k$ . Hence $||r(\varphi;a,b) - r(\psi;a,b) ||_\infty \leq \frac{L}{2} |\varphi - \psi|$ and since the range satisfies that $|\text{rg}(u)-\text{rg}(v)| \leq 2 ||u-v ||_\infty$, then:
    \begin{equation*}
        w(\varphi) - w(\psi) \leq r(\varphi;a,b) - r(\psi;a,b)  \leq L |\varphi - \psi|
    \end{equation*}
    Proving that $w$ is L-Lipchitz, as we wanted to. Now assume the minimum of $w$ over $I$ is attained at the angle $\varphi^*$, which exists by Lemma \ref{rotformulation}. By construction, some grid point $\varphi_j$ satisfies $|\varphi^* - \varphi_j| \leq h/2$, so:
    \begin{equation*}
        \tilde{\rho} \leq w(\varphi_j) \leq w(\varphi^*) + \frac{1}{2}Lh = \rho^*_I + \frac{1}{2}Lh
    \end{equation*}
    Finally, if $\rho_{lo}$ is a lower certificate of the parabolicity in $I$, then by selecting $h \leq 2 \varepsilon \rho_{lo} /L$, we obtain that $\rho \leq (1+\varepsilon)\rho^*_I$, as we wanted to prove.
\end{proof}


\subsection{Constructing the non-oriented parabolicity}

We can attempt to build a relation of a more generic parabolicity and our oriented case by defining a rotational formulation. 

\begin{lemma}[Existence of the rotational formulation] \label{rotformulation}
    For $\varphi \in [0, 2\pi)$ let $R_{\varphi}$ denote the rotation of the plane $XY$ by an angle $\varphi$, where the rotation of a given point is given by $R_{\varphi}(x_k,y_k) = (x_k(\varphi), y_k(\varphi))$ and let
    \begin{equation*}
        w(\varphi) = \rho_o(R_\varphi \mathcal{P})
    \end{equation*}
    be the oriented parabolicity of the rotated point set $\mathcal{P}$ inside the new frame of reference $X'Y'$. Let $I\subseteq [0,2\pi)$ be a closed interval such that for every $\varphi \in I$, the values $x_1(\varphi),\dots,x_n(\varphi)$ take at least three distinct values. Then $w$ is continuous on I and attains its minimum on $I$.
\end{lemma}

\begin{proof}
    Write the residual $r_k = y_k - ax_k(\varphi)^2 - bx_k(\varphi)$ and the min-max formulation of our problem using said residuals as:
    \begin{equation*}
        F(\varphi;a,b) = \max_{1\leq k \leq n}{r_k(\varphi;a,b)} - \min_{1\leq k \leq n}{r_k(\varphi;a,b)}
    \end{equation*}
    so that $w(\varphi) = \inf_{(a,b) \in \mathbb{R}^2} F(\varphi;a,b)$. Since there is a finite number of functions $r_k-r_l$, each of which is continuous in $\varphi$ and linear in $(a,b)$, the function $F$ is continuous on $I\times \mathbb{R}^2 $.
    Now, let us denote the range function of a vector in $\mathbb{R}^n$ as $\text{rg}(u) = \max_k{u_k} - \min_k{u_k}$. This function is non-negative, positively homogeneous of degree 1--that is, it satisfies that $\text{rg}(\lambda u) = \lambda \, \text{rg}(u)$ for a scalar $\lambda >0$--it is sub-additive and is zero on constant vectors, so $\text{rg} (u+v) \geq \text{rg} (u) - \text{rg} (v)$ is true. Now we define the quantity:
    \begin{equation*}
        m(\varphi) = \min_{a^2+b^2=1} {\text{rg} \left(ax_k(\varphi)^2 + bx_k(\varphi)\right)_{k=1}^n}
    \end{equation*}
    If $m(\varphi)=0$, this means there is a quadratic $ax^2+bx$ that takes constant values at every $x_k(\varphi)$. However, by the conditions imposed on $a,b$, the given quadratic function can only attain the same value at most in two different points. By assumption, we said that for any given angle $\varphi$, there would be at least three distinct $x_1(\varphi),\dots,x_n(\varphi)$, so this is a contradiction and $m(\varphi)$ is strictly positive. Since $m$ is also continuous, being the minimum of a continuous function over the compact set of the unit circle, the compactness of our interval $I$ proves the existence of a positive minimum $m_0$ of our function $m$ on $I$.

    We now define $R = \max_{\varphi \in I} {\text{rg}(y_k(\varphi))_{k=1}^n}$. We know $R$ is finite following a similar reasoning above, using the compactness of $I$ and the continuity of the maximum of a continuous function. With this, we can find a lower bound for our initial min-max formulation of the rotational problem $F(\varphi;a,b)$:
    \begin{align*}
        F(\varphi;a,b) &= \text{rg}\left(y_k - (ax_k(\varphi)^2 + bx_k(\varphi))\right)_{k=1}^n \geq \text{rg}(ax_k(\varphi)^2 + bx_k(\varphi))_{k=1}^n - \text{rg}(y_k)_{k=1}^n \\
        &\geq \|(a,b)\| m(\varphi) - \text{rg}(y_k)_{k=1}^n \geq \|(a,b)\| m_0 - R 
    \end{align*}
    Where $\|(a,b)\|$ is the Euclidean norm of $(a,b) \in \mathbb{R}^2$. And since $F(\varphi;0,0) = \text{rg}(y_k)_{k=1}^n \leq R$, then every minimizer of $F(\varphi,\cdot)$ satisfies that $\|(a,b)\|\leq 2R/m_0 = \kappa $. Therefore our oriented parabolicity can be rewritten as:
    \begin{equation}
        w(\varphi) = \min_{\|(a,b)\| \leq \kappa} {F(\varphi;a,b)} \quad \text{for every } \varphi \in I
    \end{equation}
    is a minimum of a continuous function over a compact set, and is attained. Finally, F is uniformly continuous on the compact set $I \times \{\|(a,b)\| \leq \kappa\}$ so $w$ is continuous on $I$ and Weierstrass' theorem ensures that there exists a minimizer $\varphi^* \in I$.
\end{proof}



\subsection{Upper and lower boundary support points (IGNORE)}
Even under the framework of Linear Programming and reduced computational complexity, experimental data usually contain thousands of points, which makes it necessary to reduce the number of constraints that define a problem.

Since the oriented problem in two dimensions has four degrees of freedom, for non-degenerate cases, the minimum parabolicity configuration is determined by four support points. With non-oriented cases, this can go up to five, or six, depending on whether any additional assumptions are made.

We present in this section a characterization of candidate support points for lower boundaries and an approximation of said set for upper boundaries.

\textbf{Characterization of lower boundary conditions for oriented cases.}

The following remark applies since oriented parabolas in the $XY$ plane are convex functions when $a>0$. If $a<0$, then the lemma is equivalently applied, noting the lower support points should now be considered from the direction $y=\infty$.

\begin{lemma}[Lower support points lie on the convex hull]\label{lem:lowerSupport}
Let $\mathcal{P}=\{(x_k,y_k)\}_{k=1}^{n}$ be a finite point set and let $p$ be a
convex function with
\begin{equation*}
    y_k \;\ge\; p(x_k), \qquad k=1,\dots,n .
\end{equation*}
If the constraint is active at the index $j$, that is $y_j=p(x_j)$, then
$(x_j,y_j)$ lies on the convex hull of $\mathcal{P}$. If $p$ is strictly
convex, $(x_j,y_j)$ is a vertex of that hull.
\end{lemma}

\begin{proof}
Suppose $(x_j,y_j)$ did not lie on the convex hull of $\mathcal{P}$. Then
there are indices $i,l$ and a scalar $\lambda\in(0,1)$ with
$x_j=\lambda x_i+(1-\lambda)x_l$ and
$\lambda y_i+(1-\lambda)y_l<y_j$. Using first the convexity of $p$ and then the
feasibility of the remaining two points:
\begin{equation*}
    p(x_j) \leq \lambda\,p(x_i)+(1-\lambda)\,p(x_l)
    \leq \lambda y_i+(1-\lambda)y_l
    < y_j ,
\end{equation*}
which contradicts $y_j=p(x_j)$. Therefore $(x_j,y_j)$ must be on the convex hull. If
$p$ is strictly convex, the first inequality is strict, so the same computation
with $(x_j,y_j)$ on an edge of the hull, where
$\lambda y_i+(1-\lambda)y_l=y_j$, again gives $p(x_j)<y_j$, meaning the active point is a vertex.
\end{proof}


\textbf{Approximate reduction of the upper boundary constraints for oriented cases.}

Although the convexity of parabolas imposes certain geometric restrictions on feasible support pairs and triplets, these properties were insufficient to derive a complete characterization of the upper support set. In particular, unlike the lower boundary, no criterion was identified that allows support points to be determined solely from the geometry of the point cloud. Optimal solutions may have a variable number of upper support points, ranging from a single active point to several simultaneous support points. In particular, single upper support point cases can become especially difficult to characterize, as they rely on the global geometry of the problem.

For this reason, an approximate constraint-reduction procedure is adopted. This approach is motivated by two assumptions. First, the experimental datasets considered in this work are dense, making it reasonable to replace the full point set with a reduced set of representative candidates by applying some local selection methods. Second, the data are assumed to already exhibit a parabolic-corridor structure, with the optimization affecting mainly the corridor width rather than its overall geometry. 

We approximate the candidate upper support set through a binning procedure. Let our point cloud $\mathcal{P}$ be partitioned into intervals $I_j$ along the horizontal axis. Within each interval, only the point with the maximum ordinate is retained as a candidate upper support point. Through this procedure we can achieve a controllable reduction in the number of constraints. As the bin width decreases, the candidate set approaches the original point set $\mathcal{P}$, with equality attained in the limit up to points sharing the same abscissa. Therefore, the approximation can be made arbitrarily fine while substantially reducing the computational burden for dense datasets.


\begin{figure}[h]
    \centering
    \input{binning.tex}
    \caption{Example of upper point selection}
\end{figure}


The limitations of this approximation become more apparent in the non-oriented case, where no preferred coordinate system is available and the distinction between abscissa and ordinate depends on the orientation of the candidate solution.


We have considered two possible defects in our parabolic troughs.


%%%%
Measuring errors in the data set by sections.

If the parabolicity measure obtained from any of the given points above exceeds a certain threshold, it could make sense to delve into possible errors. After all, parabolic troughs are often large in size yet fragmented into multiple separate panels that can fail individually. 

If our original algorithm, broadly speaking, has the following form:
\begin{equation} 
    \begin{split}
    &\mathrm{min} \quad \varepsilon  \\[1pt] % if you need space between objectif and constraints
    &\mathrm{s.t.} \quad 
    \begin{array}[t]{r c r}
         Ax & \leq & b\\
     \end{array}
     \end{split}
\end{equation}


And returns $\varepsilon^*$ as a result. With the related arguments $x^*$, we can then compute a local parabolicity $\varepsilon_{n,m}$ in our gridded space of $n \times m$ cells, by the new linear problem:
\begin{equation}
        \begin{split}
    &\mathrm{min} \quad \varepsilon + \lambda \Vert x-x^*\Vert_1  \\[2pt] % if you need space between objectif and constraints
    &\mathrm{s.t.} \quad 
    \begin{array}[t]{r c r}
         Ax & \leq & b\\
     \end{array}
     \end{split}
\end{equation}
This way, we can determine failures in local areas rather than in the parabolic cylinder as a whole. 




==> null_hypothesis.tex <==
\begin{tikzpicture}

% Parameters
\def\f{3}      % focal length
\def\r{1}    % circle radius

% Axes
% \draw[->, dashed] (-5,0) -- (5,0) node[right] {$x$};
% \draw[->, dashed] (0,-0.5) -- (0,4) node[above] {$y$};

% Parabola y = x^2/(4f)
\draw[ultra thick,domain=-5:5,samples=200]
    plot (\x,{(\x)^2/(4*\f)});


% Parabola y = x^2/(4f) upper bound
\draw[ultra thick, dashed, domain=-5:5,samples=100]
    plot (\x,{(\x)^2/(4*\f) + \r});

% Parabola y = x^2/(4f) lower bound
\draw[ultra thick, dashed, domain=-5:5,samples=100]
    plot (\x,{(\x)^2/(4*\f) - \r});


% Focus
%\fill (0,\f) circle (2pt);
%\node[xshift=-5pt,yshift=5pt] at (0,\f) {$F$};

% Point
\fill (1,{1/(4*\f)}) circle (2pt);

\draw[<->, thick] (1,{1/(4*\f) + \r}) -- (1,{1/(4*\f) - \r});
\node[xshift=-3pt,yshift=1pt] at (1,{(1/4*\f)}) {$2\theta$};

% Circle centered at focus
\draw[ thick] (1,{1/(4*\f)}) circle (\r);

% Point on parabola
\coordinate (P) at (5,{25/(4*\f)});
% \fill (P) circle (2pt);
% \node[right] at (P) {$P$};


% Line from focus to point
%\draw[thick] (0,\f) -- (P);
%\draw[dashed, thick] (0.15,{\f + \r -0.03}) -- (P);
%\draw[dashed, thick] (-0.1,\f - \r) -- (P);





\end{tikzpicture}


==> old_intro.tex <==

The global transition toward a decarbonized energy infrastructure requires renewable energy systems that are not only sustainable but also dispatchable. While photovoltaic (PV) and wind power generation have experienced rapid deployment, their inherent intermittency poses severe challenges for electrical grid stability. Concentrated Solar Power (CSP) technology addresses this limitation by integrating thermal energy storage systems, allowing solar energy to be stored as high-temperature heat and dispatched during periods of low solar irradiance or peak consumer demand.

A CSP facility operates by concentrating direct normal irradiance onto a central receiver or an absorber tube using extensive arrays of reflective optics, such as parabolic trough collectors (PTCs) or tower heliostats. The concentrated solar flux heats a heat transfer fluid  or molten salt mixture, which drives a conventional power block. Consequently, CSP serves as a crucial bridge between variable non-synchronous generation and stable, continuous grid operations.





%\subsection{Parabolic trough collectors}

Parabolic trough collectors are widely used in concentrated solar power (CSP) systems due to their ability to focus direct solar radiation onto a linear receiver tube. 
See Figure \ref{fig:intro}.

\begin{figure}[thb]
\centering
\begin{subfigure}{.52\textwidth}
%\centering
\includegraphics[scale =1.0]{figures/PTGeneral_real.png}
\caption{A component in a CSP.}
\end{subfigure}%
\begin{subfigure}{.40\textwidth}
%\centering
\includegraphics[scale =.14]{figures/PTGeneral.png}
\caption{Tube and reflector.}
\end{subfigure}%
\caption{Parabolic trough collector.}
\label{fig:intro}
\end{figure}




Their optical performance depends critically on the accuracy of the reflector geometry. Even small deviations from the ideal parabolic shape can lead to significant reductions in optical efficiency, caused by the misdirection of reflected rays and reduced intercept of the receiver tube. In practice, such deviations arise from multiple factors, such as manufacturing tolerances, gravitational sag, and long-term structural deformation.
Accurate characterization of these geometric deviations then becomes essential for both performance assessment and maintenance of large-scale solar fields. 
%Traditional optical evaluation methods, such as ray-tracing combined with idealized geometric models, are sensitive to assumptions about surface quality and often require simplified representations of real structural behavior. More direct geometric measurement approaches, including laser scanning and photogrammetry, provide dense spatial data that can be used to reconstruct the actual reflector surface in situ.



In industrial metrology, the problem of quantifying deviation from an ideal reference geometry is well established. Geometric dimensioning and tolerancing defines a set of form tolerances that describe how far a manufactured object deviates from its nominal shape. A representative example is cylindricity, which measures the extent to which a surface deviates from a perfect cylinder. In cylindricity evaluation, the measured surface is compared to an ideal reference cylinder, typically determined through a best-fit procedure that minimizes overall deviation. The resulting residual field provides a quantitative description of form error independent of rigid-body translations and rotations.

This concept of evaluating deviations relative to an ideal reference geometry is not limited to cylindrical or prismatic parts. It is a general principle of surface metrology that can be extended to more complex freeform shapes. Parabolic trough collectors represent a particularly relevant case, as their ideal geometry is defined by a quadratic surface rather than a simple analytic primitive such as a cylinder or sphere. Consequently, the same metrological framework can be generalized by replacing the reference cylinder with a reference paraboloid.

In this work, we adopt this perspective and treat the parabolic trough surface as a nominal quadratic reference geometry. The measured surface obtained from laser scanned point clouds is aligned to an ideal paraboloid through a best-fit optimization procedure. The deviation between the measured and fitted surfaces defines a residual field, which represents the geometric form error of the reflector. This residual field captures the combined effects of sagging, torsional deformation, manufacturing imperfections, and assembly misalignments.

By interpreting the trough surface in terms of form deviation, the problem becomes analogous to classical surface metrology problems such as cylindricity, flatness, and profile tolerance. This analogy enables the use of established mathematical tools for surface fitting, residual analysis, and statistical characterization of form error. In particular, LiDAR-derived point clouds provide a practical measurement basis for large-scale solar installations, where traditional coordinate measuring machines are not applicable.

While traditional shape detection algorithms focus on primitive geometric classification (e.g., lines, circles, ellipses, or general quadrics), solar thermal applications require a dedicated, highly specialized geometric metric which we introduce in this work as the concept of \emph{parabolicity}.
This introduces a challenging non-convex optimization landscape, giving rise to a novel class of problems in computational geometry. Solving for parabolicity under noisy, incomplete sensor sampling requires specialized algorithm design, non-linear algebraic distance metrics, and robust optimization techniques.

\subsubsection{Geometric properties of parabolic shapes (resumir)}

The fundamentals behind parabolic trough collectors rely on the basic geometry of a parabola. Their efficiency relies on the assumption that the sun as a light source is distant enough that it will always cast parallel rays in the direction determined by the solar elevation. When light hits the surface of a parabola in an ideal angle —that is, parallel to its axis of symmetry— all rays will be deflected towards the focus point. 

A diagram of the cross section of the parabolic trough is shown in Figure \ref{fig:sectionDiagram}, where we identify the main elements.

\begin{figure}[h]
    \centering
    \input{geometry_section.tex}
    \caption{Section of the parabolic trough collector}
    \label{fig:sectionDiagram}
\end{figure}

Where the following parameters are used:

\begin{itemize}
    \item $F$ as the geometric focus of the parabola. In our diagram it is located in the position $(0,f)$, with $f$ being the focal length.
    \item $V$ as the vertex of the parabola. The distance between $V$ and $F$ is the focal length.
    \item $d$ as the diameter of the receiver tube.
    \item $\theta_a$ as the acceptance half-angle. It defines the
    maximum angle relative to the axis of symmetry that the incoming rays can enter with and still be absorbed by the collector tube.
    \item $\theta_r$ as the rim angle, that is, the angle between the edge of the collector and centerline or axis of symmetry of the parabola.
\end{itemize}

Due to the typically small angles of parabolic collectors, which do not tend to exceed 2\textdegree, precise sun tracking becomes essential. Similarly, the correct reflection of sun rays is highly dependent on the collector geometry. Imperfections on the surface, causing slope errors, can quickly degrade the performance of parabolic trough solar collectors.


%The objective of this approach is to establish a simple yet robust framework for quantifying parabolic trough deformation using geometric residuals relative to an ideal reference paraboloid. Such a framework provides a bridge between structural deformation analysis and optical performance degradation, enabling systematic classification of defects such as global sagging, torsional twist, and localized panel misalignment.

%\subsection{Identifying mirror defects in PCTs}

